Adversarial Contextual Bandits Go Kernelized

We study a generalization of the problem of online learning in adversarial linear contextual bandits by incorporating loss functions that belong to a reproducing kernel Hilbert space, which allows for a more flexible modeling of complex decision-making scenarios. We propose a computationally efficient algorithm that makes use of a new optimistically biased estimator for the loss functions and achieves near-optimal regret guarantees under a variety of eigenvalue decay assumptions made on the underlying kernel. Specifically, under the assumption of polynomial eigendecay with exponent $c>1$, the regret is $\widetilde{O}(KT^{\frac{1}{2}(1+\frac{1}{c})})$, where $T$ denotes the number of rounds and $K$ the number of actions. Furthermore, when the eigendecay follows an exponential pattern, we achieve an even tighter regret bound of $\widetilde{O}(\sqrt{T})$. These rates match the lower bounds in all special cases where lower bounds are known at all, and match the best known upper bounds available for the more well-studied stochastic counterpart of our problem.

==> optimism.tex <==
%\section{Dilated bonuses}
Bounding the regularization term:

\gcomment{UPDATE THIS; I am not sure where the stray $\varepsilon$ and $\frac{\beta}{\gamma}\varepsilon$ terms came 
from in this bound...} \julia{should be fine now}
\begin{lemma}\label{l:reg_term} For any positive $\eta, \beta, M, \varepsilon$,  \kerlinexp guarantees
		%\begin{align*}\redd{
		%\widetilde{R}_T\le \frac{K \ln T}{\eta} + 2 + \epsilon + \frac{\beta}{\gamma} + 2\eta K (1+m(\epsilon ) + 
%M\epsilon)T + 2 \eta \pa{\frac{\beta}{\gamma} \epsilon + (m(\epsilon ) + M\epsilon )K}T.}
    \begin{align*}
    \widetilde R_{T} \le \frac{K \ln T}{\eta} +  2 + 2\beta(M+1) + \frac{2}{\beta v(M+1)} + 2 \eta KT \pa{ 2
 +  \pa{m(\varepsilon ) + M\varepsilon}} \cdot\pa{2+\beta^2 M}.
	\end{align*}
\end{lemma}
\begin{proof}
Let us fix $x\in\X$ and apply Lemma~\ref{l:log_barrier} to obtain the following:
	\begin{equation}
	\begin{split}
	\label{eq:regret_decomp}
		&\sum_{t = 1}^T \sum_{a\in\A} (\pi_t(a|x) - \pi^*(a|x))\pa{\hat{\ell}_k(a,x) - b_t(a,x)} \le 
\frac{\Psi(\tilde\pi^*(\cdot|x)) - \Psi(\pi_1(\cdot|x))}{\eta} +\\
		& \qquad \sum_{t=1}^T \sum_{a\in\A} ( \tilde\pi^*(a|x)  -   \pi^*(a|x) )\pa{ \hloss_t(  x,a) - b_t(x,a)  }  + \\
		& \qquad \eta \sum_{t=1}^T \sum_{a\in\A} \pi_t(a|x)\pa{ \hloss_t(  x,a) - b_t(x,a)  }^2.
		\end{split}
\end{equation}
	By picking $\tilde\pi^*(a|x) = \pa{1 - \frac{K}{T}}\pi^*(a|x) + \frac{1}{T}$, the first term is bounded by 
	\begin{align*}
		 \frac{\Psi(\tilde\pi^*(\cdot|x)) - \Psi(\pi_1(\cdot|x))}{\eta}  \le \frac{A \ln T}{\eta}.
	\end{align*}
	To proceed, we appeal to Lemma~\ref{lem:trace_M} to show that
	\[
	 	 	\bigl|\EEtb{\hloss_t(x,a)} - \loss_t(x,a)\bigr| \le \beta\EEt{\norm{\varphi(x)}^2_{ 
\widehat{\Sigma}_{t,a}^{+}}} + \frac{1}{\beta v(M+1)} = \EEt{b_{t,a}(x)} + \frac{1}{\beta v(M+1)},
	\]
	and also observe that the exploration bonus can be bounded as
	\[
	 b_{t,a}(x) = \beta \norm{\varphi(x)}^2_{\hat{\Sigma}_{t,a}^+} \le \beta \norm{\hat{\Sigma}_{t,a}^+}_2  \le 
\beta (M+1).
	\]
	Altogether, we use these observations to bound the second term in Equation~\eqref{eq:regret_decomp} as
	\begin{align*}
		 &\EE{\sum_{t=1}^T \sum_{a\in\A} ( \tilde\pi^*(a|x)  -   \pi^*(a|x) )\pa{ \hloss_t(  x,a) - b_t(x,a)  }} 
		 \\
		 &\qquad = \EE{ 
\sum_{t=1}^T \sum_{a\in\A} \frac {K\pi^*(a|x) - 1}{T}\pa{b_t(x,a) - \hloss_t(  x,a)}}
\\
&\qquad 
 \le \sum_{t=1}^T \sum_{a\in\A} \frac {K\pi^*(a|x) + 1}{T} \pa{1 + \beta(M+1) + \frac{1}{\beta v(M+1)}} 
 \\
 &\qquad = 
 2\pa{1 + \beta(M+1) + \frac{1}{\beta v(M+1)}},
	\end{align*}
	where we have used our assumption that $|\ell_t(x,a)| \le 1$ in the third line.
	
	It remains to bound the last term Equation~\eqref{eq:regret_decomp}, which we start by writing
	\begin{align*}
		&\eta \sum_{t=1}^T \sum_{a\in\A} \pi_t(a|x)\pa{ \hloss_t(  x,a) - b_t(x,a)  }^2\\
		&\le 2\eta  \sum_{t=1}^T \sum_{a\in\A} \pi_t(a|x)\pa{ \hloss_t(  x,a)  }^2 +  2\eta  \sum_{t=1}^T \sum_{a\in\A} \pi_t(a|x)\pa{ b_t(  x,a)  }^2.
	\end{align*}
	We will bound this term on expectation with respect to the random context $X_0$ drawn independently from the 
interaction history between the learner and the environment.
The first term in the resulting expression can be upper bounded by using Lemma~\ref{l:variance}:
			$$\EEt{\sum_{t=1}^T\sum_{a=1}^A   \pi_t(a|\tX)   \biprod{\varphi(\tX)}{\wt{f}_{t,a}}^2} \le  2K \pa{ 1  +  (m(\varepsilon ) + 
M\varepsilon)}.$$
	Moving on to the second term, we have
	\begin{align*}
		&\EEt{ \sum_{t=1}^T \sum_{a\in\A} \pi_t(a|\tX)\pa{ b_t(  \tX,a)  }^2} = \beta^2 \EEt{ \sum_{t=1}^T \sum_{a\in\A} 
\pi_t(a|\tX) \norm{\varphi(X_0)}_{\hSigma^+_{t,a}}^4} \\
		& \le  \beta^2 M  \EEt{ \sum_{t=1}^T \sum_{a\in\A} \pi_t(a|\tX) \norm{\varphi(X_0)}_{\hSigma^+_{t,a}}^2}\\
		&\le  \beta^2 M\EEt{ \sum_{t=1}^T \sum_{a\in\A}  \trace{\Sigma_{t,a} \hSigma^+_{t,a} }}\\
		& \le \beta^2 M  \pa{m(\epsilon) + M\epsilon} KT,
	\end{align*}
	where the last inequality uses Lemma~\ref{lem:effective_dim_MGR}. Collecting all terms together, we get
	\begin{align*}
	\widetilde R_{T} \le \frac{K \ln T}{\eta} +  2 + 2\beta(M+1) + \frac{2}{\beta v(M+1)} + 2 \eta KT \pa{ 2
 +  \pa{m(\varepsilon ) + M\varepsilon}} \cdot\pa{2+\beta^2 M},
\end{align*}
thus concluding the proof.
\end{proof}	

\paragraph{Proof of  Theorem~\ref{th_robust_kernel}.}
Using Lemma~\ref{lem:trace_M}, we have
\begin{align*}
	 \EE{B_T} + \EE{B^*_T} & \le   \beta \sum_{t=1}^{T} \EE{ \sum_{a\in\A}  \pa{\pi_t(a|X_0) +\pi^*(a|X_t)}
\norm{\varphi(X_0)}^2_{ \widehat{\Sigma}_{t,a}^{+}} } +\frac{2}{\beta v(M+1)}
\\
& =   \sum_{t=1}^{T} \EE{ \sum_{a\in\A}  \pa{\pi_t(a|X_0) +\pi^*(a|X_t)}
b_{t,a}(X_0)} +\frac{2}{\beta v(M+1)}
\end{align*}
Therefore, by plugging this bound into the regret decomposition of Equation~\eqref{eq:regret_dec}, we obtain
\begin{align*}
	R_T \le& \widetilde{R}_T +   \sum_{t=1}^{T} \EE{ \sum_{a\in\A}  \pa{\pi_t(a|X_0) +\pi^*(a|X_t)}
b_{t,a}(X_0)} +\frac{2}{\beta v(M+1)} 
	\\
	&\qquad+ \sum_{t=1}^{T} \EE{\sum_{a\in\A} (\pi_{t}(a|\tX) - \pi^*(a|\tX)) b_{t,a}(X_0)}\\
	\le&   \widetilde{R}_T +   2 \sum_{t=1}^{T} \EE{ \sum_{a\in\A}  \pi_t(a|X_0) b_{t,a}(X_0)} +\frac{2T}{\beta 
v(M+1)}.
\end{align*}
\gcomment{This comment is misplaced: This is why the bonus term $b_t(x,a)$ is useful - it allows to cancel the 
problematic term $\EE{   \pi^*(a|X_0) \norm{\varphi(X_0)}^2_{ \widehat{\Sigma}_{t,a}^{+}} } $. }
The second term above can be bounded by appealing to Lemma~\ref{lem:effective_dim_MGR} as
\begin{align*}
	 \EE{  \pi_t(a|X_0) \norm{\varphi(X_0)}^2_{ \widehat{\Sigma}_{t,a}^{+}} } =  \EE{\trace{\Sigma_{t,a} 
\widehat{\Sigma}_{t,a}^{+} }}  \le m(\epsilon) + 
M\epsilon. 
\end{align*}
Appealing to Lemma~\ref{l:reg_term} to bound $\wt{R}_T$ and collecting all terms together, we get ........... 
\gcomment{Somebody sane please do these calculations}
\begin{align*}
    R_T \le \frac{K \ln T}{\eta} +  2 + 2\beta(M+1) + \frac{2}{\beta v(M+1)} + 2 \eta KT \pa{ 2
 +  \pa{m(\varepsilon ) + M\varepsilon}} \cdot\pa{2+\beta^2 M} \\
 + \frac{2T}{\beta v (M+1) } + 2\beta K (m(\varepsilon)+M\epsilon)T.
\end{align*}


% \begin{align*}
% 	R_T &\le \frac{K \ln T}{\eta} +  \frac{\beta}{\gamma} + \frac{\gamma}{\beta}+\delta + 2 \eta T  A \pa{ 1  +  
%(m(\varepsilon ) + \frac{\varepsilon}{\gamma})} + 2 \eta  \beta^2 M A \delta T + 2\eta \beta^2 M  AT (m(\epsilon) + 
%\frac{\epsilon}{\gamma}) \\
% 	&+ 2\beta TA \pa{ \frac{\gamma}{\beta} + \delta  + \delta \frac{\beta}{4}} + 2 \beta T A \pa{m(\epsilon) + \frac{\epsilon}{\gamma} + \delta} 
% \end{align*}

%To simplify the analysis, take $M= \frac{2\log( 1/\gamma)}{\gamma}$, $ \beta: = \eta$, $\delta := \gamma$, which gives:
% \begin{align*}
%	R_T &\le \frac{A \ln T}{\eta} +  \frac{\eta}{\gamma} + \frac{\gamma}{\eta}+\gamma + 2 \eta T  A \pa{ 1  +  2m(\varepsilon ) + 2\frac{\varepsilon}{\gamma} + 2\gamma + \frac{\gamma}{\eta}   + \gamma\frac{\eta}{4}} + 4 \eta^3 A  T \frac{\log( 1/\gamma) }{\gamma}  +\\
%	&  2\eta^3   \frac{2\log( 1/\gamma)}{\gamma}AT (m(\epsilon) + \frac{\epsilon}{\gamma}).
%\end{align*}

 We will tune the parameters $\eta, \beta, \epsilon, M$ independently for different eigendecays regime. Consider the polynomial  eigenvalues decay rate $\mu_i  \le g i^{-c}$. Then,  $\varepsilon= \sum_{i=m+1}^{\infty} \mu_i \le g m^{1-c}$. Taking $m = T^{\frac{1}{c}}$, $M = T$, $\eta = \beta = T^{-\frac{1}{2}\pa{1+\frac{1}{c}}}$ the expected
 	regret of \kerlinexp  satisfies
 	\begin{align*}
 		R_T = \OO\pa{ A \sqrt{ \log(T)}  T^{\frac{1}{2} \pa{1+\frac{1}{p}}}}.
 	\end{align*}
 	
 	For the exponential decay $\mu_i  \le C e^{-c i}$, $\varepsilon \le C e^{-c m}$. So, taking $m = \log T/ c$, $M = T$, $\eta = \beta = T^{-1/2}$, we get 
 	\begin{align*}
 		R_T = \OO\pa{   A\sqrt{T} \log(T) }.
 	\end{align*}


\qed
